Improving the Inference of Topic Models via Infinite Latent State Replications

In text mining, topic models are a type of probabilistic generative models for inferring latent semantic topics from text corpus. One of the most popular inference approaches to topic models is perhaps collapsed Gibbs sampling (CGS), which typically samples one single topic label for each observed document-word pair. In this paper, we aim at improving the inference of CGS for topic models. We propose to leverage state augmentation technique by maximizing the number of topic samples to infinity, and then develop a new inference approach, called infinite latent state replication (ILR), to generate robust soft topic assignment for each given document-word pair. Experimental results on the publicly available datasets show that ILR outperforms CGS for inference of existing established topic models.

==> 3.Preliminaries_ICDM.tex <==
~\section{Preliminaries}
\label{sec:preliminaries}
%\begin{table}[t]
%  \caption{Notation}
%  \label{tab:notation}
%  \centering
%  \begin{tabular}{lm{5.8cm}}
%    \toprule
%     %\multicolumn{2}{c}{Inference methods} &  \multicolumn{2}{c}{LDA}\\
%     %\cmidrule(l{2pt}l{2pt}){1-2}  \cmidrule(l{2pt}l{2pt}){1-2}
%    $Y$,$Z$  & Sets of random variables  \\
%    $i$ & Superscript used to indicate the $i^{th}$ iteration\\
%    $\textbf{X},\textbf{|X|}$ & Dataset of document-word pairs represented as a table\\
%    \textbf{|X|}& Number of rows in the dataset\\
%    \multirow{2}{*}{$j$,$m$} & Subscripts used to index a row in the dataset and assignments  that depend on\\
%    & that row \\
%    $x^{(d)}_j,x^{(w)}_j$ & Document and word stored at the $j^{th}$ row in the dataset \\
%    $K$ & Number of topics\\
%    $Z_j$, $Y_j$  & Random variables assigned to the pair $(x^{(d)}_j,x^{(w)}_j)$\\
%    $Z_{-j}$,$Y_{-j}$ & Sets of random variables excluding the $j^{th}$ random variable\\
%    \multirow{2}{*}{$Z_{>j}$,$Z_{<j}$ } & Sets of random variables assigned to the records whose indices are greater\\
%     &than $j$ and lesser than $j$ respectively\\
%    $z_j$ & Realization of a random variable $Z_j$. $z_j$ uses a one-hot encoded representation\\
%    $R_{Z_j}$ & Support of a random variable\\
%    $R_{Z_{-j}}$ & Support of the joint distribution composed by $Z_{-j}$  \\
%    $p(Z_{j}|Z_{-j},\textbf{X})$ & Posterior distribution used to sample the topic assignment of the pair $(x^{(d)}_j,x^{(w)}_j)$\\
%    $\eta_j$ & Parameters of $p(Z_j|Z_{-j},\textbf{X})$\\
%    $\eta_{-j}$ & Set of parameters of all posterior distributions excluding  $\eta_j$ \\
%    $f_{Z_{j}|Z_{-j}}(z)$ & Probability density of  $p(Z_{j}|Z_{-j},\textbf{X})$\\
%    $D_{x^{(d)}_j}$,$W_{x^{(w)}_j}$,$N_j$ & Statistics used to compute $f_{Z_{j}|Z_{-j},\textbf{X}}(z)$\\
    %\multirow{2}{*}{g(X)}&The function g() transforms a categorically distributed \\
    %&random variable into a degenerate-Dirichlet random variable\\
%    \bottomrule
%  \end{tabular}
%\end{table}

%We define the main notations used throughout this paper in Table \ref{tab:notation}. %Note that $p(X)$ is the probability distribution of $X$ and not the probability of $X$.

%\subsection{Latent Dirichlet Allocation via Collapsed Gibbs Sampling}

Latent Dirichlet allocation (LDA), one of the most common topic models, is able to discover $K$ topics that pervade an unstructured collection of documents. In LDA, we assume that each document has a multinomial distribution over $K$ topics parameterized by $\theta$. We use $\theta_{d}$ as the parameter for representing $p(Z|d)$, the probability distribution of the topics in a document $d$. Each topic is defined as a multinomial distribution over the vocabulary of words parameterized by $\phi$. We use $\phi_{w}$ as the parameter for representing $p(w|Z)$, the probability of observing the word $w$ given a topic. The per document topic distribution $\theta_d$ is generated by sampling from a Dirichlet distribution with hyper-parameters $\alpha$, and the per topic word distribution $\phi_w$ is generated by sampling from a Dirichlet distribution with hyper-parameters $\beta$.

In latent Dirichlet allocation via collapsed Gibbs sampling (LDA-CGS), 
to find latent topics, we use a dataset $X$ consisting of $M$ document-word pairs $x_j=(x_j^{(d)},x_j^{(w)}) ~\forall j \in 1 \cdots M$, where $d$ indexes one of the documents, and $w$ indexes a word in the vocabulary with size $V$. Each pair is assigned exactly to one of the topics as established by the assumptions of the model. The topic assignment is generated by sampling the conditional posterior distributions of the topic assignment $Z_j$ of the $j^{th}$ pair given the topic assignments of all other pairs $Z_{-j}=z_{-j}$. Formally, we represent the conditional posterior distribution as $p(Z_j|Z_{-j}=z_{-j},\textbf{X})$. The probability density of the posterior distribution is given in Equation \ref{eq:ldacgs}.

\begin{equation}
\label{eq:ldacgs}
f(Z_j|Z_{-j}=z_{-j}) \propto \frac{(D_{x^{(d)}_j}+ \alpha) (W_{x^{(w)}_j}+\beta)}{(N_j+V\beta)}
\end{equation}

We use the subscript $Z_j|Z_{-j}$ to denote the density of the posterior distribution $p(Z_j|Z_{-j},\textbf{X})$. $D_{x^{(d)}_j}, W_{x^{(w)}_j}$ and $N_j$ are count vectors computed using the indicator function $\mathds{1}()$:
\begin{gather}
\begin{align}
D_{x^{(d)}_j}={\sum_{m=1,m\neq j}^{M}}\mathds{1}(x^{(d)}_j=x^{(d)}_m)*z_m 
\end{align}\\
W_{x^{(w)}_j}={\sum_{m=1,m\neq j}^{M}}\mathds{1}(x^{(w)}_j=x^{(w)}_m)*z_m \nonumber\\
 N_j={\sum_{m=1,m\neq j}^{M}}z_m
\label{eq:factors}
\end{gather}

%https://tex.stackexchange.com/questions/238333/how-to-set-the-position-of-an-equation-in-latex?utm_medium=organic&utm_source=google_rich_qa&utm_campaign=google_rich_qa


\noindent
where $z_m$ corresponds to the realization of the random variable $Z_m$. Note that $z_j$ and $z_m$ are represented as one-hot vectors. Hence, $D_{x^{(d)}_j}$ denotes the vector of topic assignments for document $x^{(d)}_j$, $W_{x^{(w)}_j}$ denotes the vector of topic assignments for word token $x^{(w)}_j$, and $N_j$ represents the vector of topic assignments over the entire set of document-word pairs. This representation facilitates the comparison of Equation \ref{eq:ldacgs} with the posterior density proposed in Section \ref{sec:dgm}.

This collapsed Gibbs sampling for LDA (LDA-CGS) is summarized in Algorithm \ref{alg:cgs}. Note that at iteration $i$, the computation for the posterior density in line 5 not only depends on the topic assignments of all the pairs whose index values are smaller than $j$, as denoted by $z^{i}_{<j}$, but also depends on the topic assignments of all the pairs indexed with values greater than $j$ at iteration $i-1$, as denoted by $z^{i-1}_{>j}$. Thus, we denote the density at the $i^{th}$ iteration for the $j^{th}$ record to be $f(Z^i_j|Z^i_{<j}=z^i_{<j}, Z^{i-1}_{>j}=z^{i-1}_{>j})$.


\begin{algorithm}
   \caption{Collapsed Gibbs Sampling for LDA}
   \label{alg:cgs}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Hyperparameters $K,\alpha,\beta$, dataset $\textbf{X}$
   \STATE Initialize $z^0_j$ using a uniform distribution, and set initial iteration $i=1$
   \REPEAT 
   \FOR{$j=1 \cdots M$}
   \STATE Compute $f(Z^i_j|Z^i_{<j}=z^i_{<j}, Z^{i-1}_{>j}=z^{i-1}_{>j})$ from Equation\ref{eq:ldacgs}
   \STATE Draw $z_j^i$ from $f(Z^i_j|Z^i_{<j}=z^i_{<j}, Z^{i-1}_{>j}=z^{i-1}_{>j})$
   \ENDFOR
   \STATE $i=i+1$
   \UNTIL{Convergence}
   \STATE Collect samples and estimate $\hat{\theta}$ and $\hat{\phi}$ as shown in \cite{ldacgs}
   \RETURN $\hat{\theta},~\hat{\phi}$
\end{algorithmic}
\end{algorithm}

%Although the convergence is guaranteed \cite{casella}, it is hard to assess this convergence. The problem stems from sampling, because the samples represent all the information about the marginal densities hence it is hard to measure if the samples are i.i.d draws from the target marginal distributions. 

The convergence of LDA-CGS can be obtained when the topic assignments $z_j$ for each pair are drawn from the marginal distributions $p(Z_j)$. Unfortunately, since we do not have an analytical form for $p(Z_j)$, we cannot measure at which iteration the samples are drawn from $p(Z_j)$ . 

%2018!!!!!
%Typically, the algorithm is run for a large number of iterations. Then, a number of samples are stored to estimate the parameters $\theta$ and $\phi$. The samples are stored at spaced intervals to simulate independent sampling \cite{topicmodels}. These samples are all the information required to estimate the parameters of LDA.  Given $S$ samples $z^s_j ~\forall j \in 1 \dots \textbf{M} ~\forall s \in 1 \dots \textbf{S}$, for a total of $S \times M$ samples. We can estimate the parameters as:

%\begin{equation}
%\label{eq:ldacgsparams}
%\hat{\theta}_{x^{(d)}_j} \propto \dfrac{1}{S}\sum_{s=1}^{S} (D^{s}_{x^{(d)}_j}+\alpha) ~~;~~\hat{\phi}_{x^{(w)}_j} \propto \dfrac{1}{S}\sum_{s=1}^{S} (W^{s}_{x^{(w)}_j}+\alpha)
%\end{equation}

%Where $D^s_{x^{(d)}_j}$ and $W^s_{x^{(w)}_j}$ are  constructed from the samples obtained by the $s^{th}$ sampling batch.

%Although the convergence of LDA-CGS is guaranteed \cite{casella}, the assessment of convergence must be estimated and the accuracy of this estimation depends on the method used to obtain the samples as well as the number of samples taken for the estimations of $\hat{\theta}$ and $\hat{\phi}$ \cite{zellner}. 
%%end2018!!!!!

%The problem stems from sampling. The samples represent all the information about the marginal densities and it is hard to measure if the Markov chain is approximating the target marginal distributions $p(Z_j) ~\forall j \in 1 \cdots M$. In addition, the samples used on the estimations may not satisfy independent draws from the posterior distributions. % We observe that sampling is the only step preventing a natural way to implement collapsed Gibbs sampling as a deterministic algorithm. 
%To avoid sampling, we need to derive an alternative method for updating the topics. %This is the idea behind deterministic Gibbs motion as explained in the next section.


%%250818
Zhao and Canny showed that by using an augmentation of the latent state, the predictive power of the algorithm increases since the estimation approaches the maximum a posteriori \cite{SAME}. The augmentation technique corresponds to modifying the probabilistic model by adding multiple independent copies of the latent variable. In the case of LDA, the technique is applied as shown in Figure \ref{LDArep}. Intuitively, the topic assignment of LDA does not corresponds to a single label, but instead, it is assigned to a mixture of labels. 

\begin{figure}
\label{LDArep}
  \caption{LDAs}
  \centering
    \includegraphics[width=0.5\textwidth]{LDAs}
\end{figure}

From the generative perspective, the categorical distribution of $p(Z|\Theta)$ is now represented by a multinomial distribution with n trials. 

The authors derive the new posterior:

\begin{gather}
\begin{align}
D_{x^{(d)}_j}={\sum_r^R\sum_{m=1,m\neq j}^{M}}\mathds{1}(x^{(d)}_j=x^{(d)}_m)*z_m 
\end{align}\\
W_{x^{(w)}_j}={\sum_r^R\sum_{m=1,m\neq j}^{M}}\mathds{1}(x^{(w)}_j=x^{(w)}_m)*z_m \nonumber\\
 N_j={\sum_r^R\sum_{m=1,m\neq j}^{M}}z_m
\label{eq:factors}
\end{gather}
(TODO: Add  the index r inside the notation)

This new algorithm naturally increases the computational complexity by R times. Hence Zhao et al. proposed to cast the multiple trials of the multinomial into one sample of a Poisson distribution.  As explained by the authors, the generation of one Poisson sample is equivalent to the generation of up to 100 trials of the multinomial distribution. 

In this work, we show that it is possible to maximize the number of trials by raising R to infinity without incurring on extra computational complexity. Furthermore, we take a look at the case where the topics may be dependent

However clearly the cost of the algorithm is now 
up to m of 100.
However, it is not clear how can we maximize the replication to larger numbers without having to handle higher computational costs. 

Intuitively the topic assignment becomes a mixture and by increasing the flexibility of the topic assignment, the model is able to find a better estimation. After all the estimation depends exclusively on 

minor advantages are the convergence and determinism.   


In this paper we present a transformation of the latent state that empowers the inference algorithm with soft topic assignments. We use a function to transform the latent random variables from a categorical distribution, whose outcome corresponds to a topic, into degenerate Dirichlet, whose outcome corresponds to a mixture of topic assignments.




In this paper we show that it is possible to derive a formula

$p(\Theta,Z,X) \propto \prod_{r=1}^R p(\Theta^{(r)},Z,X)$

%\input{attemptderivem}

other models where it is unclear how to use the Poisson sampler to estimate the topic assignments 








==> 4.DGM.tex <==
\section{Recursively Compound Allocation}
\label{sec:dgm}


%\begin{figure*}[t]
%  \centering
%  \includegraphics[width=1.0\textwidth]{samplecompound}
%  \caption{Difference between sampling and compounding on LDA.  On the left, we show the step 5 and 6 of Algorithm \ref{eq:ldacgsparams} for the first row of the dataset. On the right, we show step 6 of Algorithm \ref{eq:ldadgmparams}. In both cases we assume K=3.}
%  \label{fig:difference}
%\end{figure*}

%Gibbs sampling is an iterative method that samples conditional distributions to obtain estimates of marginal distributions. As benefit, we avoid calculations that may be prohibited in some cases. 

%Problem of sampling: estimation of parameters, estimation of posterior

%In this section, we show that by replacing sampling conditional distributions with compounding distributions, we obtain a deterministic approach to Gibbs sampling that estimates the marginal densities directly without using samples. We show that this method inherits the same theoretical guarantees of Gibbs sampling with two extra benefits:

%\begin{enumerate}
%\item The direct estimation of the distributions facilitates the assessment of convergence which can be checked directly from the per iteration changes of the parameters.
%\item In some cases, the estimation of the model's parameters is often more granular and it is possible to obtain a more accurate estimation. We explain this benefit by applying DGM to the Latent Dirichlet Allocation in section \ref{sec:app}.
%\end{enumerate}

%% Recap on CGS
In LDA inferred by CGS, we compute the posterior distribution for an observed document-word pair by using the topic assignments of all the other pairs. Then, we rely on the posterior distribution to sample a single topic label for the pair. As argued earlier, by allowing the soft-topic assignment, i.e., directly employing the distributions of topic assignments instead of exact assignments of latent topics, we may relax the inference process and enhance the predictive power of LDA. %In addition, the samples obtained by CGS do not allow us to assess the convergence of LDA-CGS. 

%% Introduce RCA
Generally, a distribution whose parameter is again distributed according to other probability distribution is often known as compound probability distribution.
Then, in order to improve the predictive ability of CGS,
for each given document-word pair, 
%we follow the Gibbs sampling framework, 
instead of sampling the exact topic label, we propose to use the compound distribution as the soft-topic assignment. 
In other words, the posterior topic distribution for the given document-word pair will be computed directly from the distributions of topic assignments of all the other document-word pairs. 
In this way, we develop a new deterministic inference method within the Gibbs sampling framework, named recursively compound allocation (RCA). 


%% Dr. Hai June 6th
%Specifically, for given observed document-word pairs, we follow the Gibbs sampling framework, but instead of sampling exact topic labels, we propose to leverage the compound distributions of topic assignments, and then develop a deterministic method, called recursively compound allocation (RCA), for inference of latent topics.  
%In this way, the posterior topic distribution for a given document-word pair will be computed by compounding the topic distribution assignments of all the other document-word pairs. This process is known as compound distributions (?? definition not very clear ??).


%% Dan June 6th
%In LDA-CGS, we compute the posterior topic distribution
%for a document-word pair by using the topic assignments
%of all the other pairs. Then, we rely on the posterior topic
%distribution to sample a topic label for the pair. As argued
%earlier, by allowing a soft-topic assignment, we relax the
%inference process, and LDA can enhance its predictive power.
%%Our proposed method follows the Gibbs sampling frame-
%work. But instead of sampling topic label assignments, we use
%a topic distribution as the topic assignment. As consequence,
%the computation of the posterior topic distributions for one
%document-word pair will be based on the topic distributions
%assignments to all other document-word pairs. Distributions
%whose parameters are based on other distributions are known
%as compound distributions. On that perspective, we label our
%method as Recursively Compound Allocation (RCA).
%In the next subsections, we show that by selecting the
%right topic distribution, our method is able to cast a vanilla
%probabilistic topic model into a model with normalized soft-
%topic assignments. In addition, we show that our method is
%convergence-aware.


%% An analogy with EM can be found in version 1.

%In particular, the topic assignment distribution for a given pair is computed using the principle of \textit{compound distribution}, where we compound the topic assignment distributions for all the other document-word pairs to derive the distribution for the given observed pair. %that uses topic distributions of the other document-word pairs to compute the distributions of the given pair. %To motivate the need for compounded distributions, we start by introducing the problem of the assessment of convergence in Gibbs sampling and how we can use compounded distributions to solve this problem.

First, we illustrate how to transform Gibbs sampling into a deterministic process with a simplified task. 

\subsection{Transforming Gibbs Sampling into Deterministic Process}

Given a set of random variables $X_1, X_2, \cdots, X_M$, we are typically interested in estimating densities related to these random variables, e.g., the marginal densities $f(X_1), f(X_2), \cdots f(X_M)$. However, it is often the case that these distributions cannot be found analytically. 
Hence, we resort to iterative methods, such as Gibbs sampling, to estimate the marginal distributions. 
%%TODO: The following paragraph seems to be already mentioned above !!!
%Unfortunately, these samples are not sufficient for assessing the convergence %of Gibbs sampling. In our proposed method, not only there exists a clear %assessment of convergence, but we show that by allowing a distribution as the %topic assignment, the models can enhance their predictive power. 

%Let us give an example to illustrate the idea. 
Without loss of generality, we consider two random variables $X_1$ and $X_2$. As a requirement of Gibbs sampling, we assume that we know the analytical form of the conditional densities $f(X_1|X_2)$ and $f(X_2|X_1)$. Then, Gibbs sampling performs the following procedure iteratively:

\begin{center}
\begin{enumerate}
\item Select an initial sample $x^0_2$
\item Sample $x^1_1$ from $f(X_1|X_2=x^0_2)$
\item Sample $x^1_2$ from $f(X_2|X_1=x^1_1)$
\item Repeat until convergence
\end{enumerate}
\end{center}

%%Trying to fit this figure one page earlier
\begin{figure*}[t]
  \centering
\includegraphics[scale=0.7]{cat2deg3}
  \caption{Using the function $g()$ to transform an r.v. $Z_j$ with categorical distribution to an r.v. $Y_j$ with degenerate Dirichlet distribution.}
  \label{fig:cat2deg}
\end{figure*}

As the number of iterations increases, the samples $x_1$ and $x_2$ approximate to the samples from the joint distribution $f(X_1,X_2)$. Unfortunately, the exact number of iterations to convergence is unknown, since it is not possible to decide the convergence of a distribution using the samples. %we cannot quantify if the samples are drawn from the joint distribution whose analytical form is unknown.

%We cast the Gibbs sampling process into a process using soft-assignments,(technically incorrect)
We would transform CGS into the deterministic RCA, if in step 2 we do not sample $x^1_1$ from $f(X_1|X_2=x^0_2)$, but instead, we define a random variable $X^1_1$ distributed according to the density $f(X_1|X^0_2)$, where $X^0_2$ is an initial distribution assigned to $X_2$. 
Then, we use the newly defined random variable $X^1_1$ as the conditional variable to obtain the density of $X^1_2$. 
Formally, $X^1_1$ and $X^1_2$ are compound distributions, as their parameters depend on random variables, and not on sample assignments. 
To summarize,

\begin{center}
\begin{enumerate}
\item Initialize the parameters of the density for $X^0_2$
\item Define $X^1_1 \sim f(X_1|X^0_2)$
\item Define $X^1_2 \sim f(X_2|X^1_1)$
\item Reiterate until convergence.
\end{enumerate}
\end{center}


To obtain the density of $X_1^1$, we apply the principle of compound distribution \cite{casella} as follows:
\begin{equation}
\label{eq:compound}
f(X^{1}_1)= \sum_{x_2 \in R_{X^0_2}} f(X_1|X^0_2=x_2) f(X^{0}_2=x_2),
\end{equation}
where $R_{X^0_2}$ denotes the support of $X^0_2$. We can then compute $f(X^{1}_2)$ in a similar way. %We coin this idea as recursively compounded allocation (RCA), because the distribution of $X_1$ is a compound distribution that depends on the random variable $X_2$, and recursively, $X_2$ is a compound distribution that depends on the random variable $X_1$. 


Although it may seem as if the new deterministic process,
which leverages the compound distributions of topic assignments instead of particular topic labels,
converges to a different result, Gelfand and Smith showed that 
this deterministic process, also known as the substitution algorithm, converges to the desired marginal distributions of Gibbs sampling \cite{smith}. % As a matter of fact, this process is equivalent to a deterministic version of Gibbs sampling known as the substitution algorithm \cite{smith}. 

Unfortunately the substitution algorithm is in most cases intractable, specially when the number of random variables is greater than two. Assuming $M$ random variables, we have that:

\begin{equation}
\label{eq:intractable}
f(X_j|X_{-j})=\sum_{X_{-j}}f(X_j)f(X_1,\cdots X_{\neq j}, \cdots X_{M})  \hspace{-0.7em} 
\end{equation}







%use marginals to identify join

Despite the subtlety, by transforming Gibbs sampling into a deterministic process, we obtain an additional benefit of having the ability to flag the convergence status. %By using distributions to replace the hard topic assignments, 
The deterministic procedure is able to measure the distance of the assigned distributions between two given iterations. 
When this distance is smaller than a predetermined value, the method is able to specify the convergence of the inference.
%assessment can be achieved by selecting an appropriate statistical distance that is able to measure the distance between the posterior distributions.

 %, and one of its advantages is that there exist metrics which can be used to quantify if the density of the random variables $X_1$ and $X_2$ is similar to their density at the previous iteration \cite{casella}. %Hence, we can assess the convergence of the Gibbs method.
%We coin this idea as \textit{Deterministic Gibbs Motion (DGM)} because the convergence is the same as Gibbs sampling, but there is no sampling involved. 
 %distributions computed   is the same as Gibbs sampling, but there is no sampling involved. 

%Unfortunately, in most cases the probability density of $\hat{X_1}$ and $\hat{X_2}$ is analytically intractable. This is because 
%Distributions of the newly defined random variables then become \textit{compound distributions}, since the conditional variables of $f(X_1|X_2)$ and $f(X_2|X_1)$ are random variables. %The density of the compound distribution for $X_1$ can be found as:


%As we discuss in the next section, the substitution algorithm %the %deterministic approach to Gibbs sampling 
%is intractable for topic models, a convenient solution is to assign a different %topic distribution that not only allows this process to be tractable, but %coincidentally, it empowers a topic model with soft-topic assignments.


\subsection{Latent Dirichlet Allocation Inferred via RCA}

%Using the above principle, DGM computes topic distribution for the $j^{th}$ pair as follows:
Following the aforementioned steps, in this section, we transform the inference of latent Dirichlet allocation via collapsed Gibbs sampling (LDA-CGS) into a deterministic process. %we do not need to assign a topic to a document-word pair. Instead, 


First, we assign a topic distribution to the $j^{th}$ document-word pair given random variable distributed as  $\hat{Z_j} \sim p(Z_j|Z_{-j},\textbf{X})$, where $Z_{-j}$ corresponds to topic distributions of all the document-word pairs sans the $j^{th}$ pair. Since the conditionals $Z_{-j}$ are also random variables, $Z_j$ is distributed according to the following compound distribution:
\vspace{-0.5cm}

\begin{equation}
\label{eq:compoundlda}
f(Z_j|Z_{-j},X)=\sum_{Z_{-j}}f(Z_j)f(Z_1,\cdots Z_{\neq j}, \cdots Z_{M})  \hspace{-0.7em} 
\end{equation}

%Because the marginal distributions $f(Zj)$ take an analytic form, we can quantify the convergence of the distribution.
Similarly, the method applies the same equations to all other document-word pairs until their posterior distributions converge to the target distributions $P(Z_j)$ of collapsed Gibbs sampling. %2018!!! changes
 %CGS is non deterministic due to its sampling nature. The obtained samples do not allow the computation of the distance between the topic assignments of an iteration and its previous one. In contrast,
%(copied above) One benefit of RCA is that it is deterministic, simply because it does not use sampling. By using distributions to replace the hard topic assignments, RCA is able to measure the distance between iterations. The convergence assessment can be achieved by selecting an appropriate statistical distance that is able to measure the distance between the posterior distributions. %For example, the Chi-Square test.  %In addition, the estimation of the parameters can be performed without sampling using the target densities  as presented in Equation \ref{eq:ldadgmparam}.% We present the proof of convergence in Section \ref{subsec:proof}. The motion of the marginal distributions is used to coin the label of deterministic Gibbs motion. % Finally, we use a numerical example to clarify how the method works.

%\begin{equation}
%\label{eq:ldadgmparam} 
%\hat{\theta}_{x^{(d)}_j} \propto  \sum_{m=1}^{|X|}\left(\mathds{1}(x^{(d)}_j=x^{(d)}_m)f_{Z_m}(z)+\alpha \right) ~~;~~\hat{\phi}_{x^{(w)}_j} \propto  \sum_{m=1}^{|X|}\left(\mathds{1}(x^{(w)}_j=x^{(w)}_m)f_{Z_m}(z)+\beta \right)
%\end{equation}

% Note the marginals will be independent 

%We borrow the example from \cite{casella}. Given a joint density $f_{X,Y}(x,y)=\binom nx y^{x+\alpha-1}(1-y)^{n-x+\beta-1}, ~x \in \mathbb{N}_{[1,n]}, ~ 0 \leq y \leq 1$, and the values $\alpha$ and $\beta$,  we can obtain the conditional distributions required for DGM as follows:

%\begin{center}
%$p(X|Y)$ is $Binomial(n,y)$\\
%$p(Y|X)$ is $Beta(x+\alpha,n-x+\beta)$\\
%\end{center}

%Following Algorithm \ref{alg:dgm}, we initialize $Y^0 \sim Beta(\alpha,\beta)$ with initial parameters $\alpha$ and $\beta$. Then, in step 5, we define $X^1 \sim Binomial(n,Y^0)$ which is equivalent to  $X^1 \sim Beta$-$bin(n,\alpha,\beta)$. Iterating the loop at step 4, we define $Y^1 \sim Beta(X^1+\alpha)$  which transforms into $Y^1 \sim Beta(\alpha, \beta)$. At this step, we observe how the random variables $X$ and $Y$ have broken their interdependence. If we continue to iterate we would trivially obtain $X^2 \sim Beta$-$Bin(n,\alpha,\beta)$ and $Y^2 \sim Beta(\alpha,\beta)$ which further proves the algorithm has converged. In effect, we have obtained the marginal distributions of $X$ and $Y$. This example is merely illustrative since both $p(X)$ and $p(Y)$ can be computed from integrating the joint distribution. Furthermore, the choice of the initial $\alpha$ and $\beta$ is convenient, any other initialization is likely to encounter a compound distribution which is analytically intractable.

%The family of models where DGM applies is just a subset of the cases where Gibbs sampling applies. Section \ref{sec:app} discusses the family of models where DGM can be applied independent of the initialization values.

%Using Equation \ref{eq:compoundlda} we can compute the distribution assignment to the $j^{th}$ document-word pair.
Unfortunately, Equation \ref{eq:compoundlda} is intractable, as $f(Z_1,\cdots Z_{\neq j}, \cdots Z_{M})$ is analytically unknown.
% as it involves at least $K^{M-1}$ summation terms. %This equation is harder to compute than its CGS counterpart presented in Equation \ref{eq:ldacgs}. %Therefore, DGM sacrifices the computational complexity of the Gibbs method for allowing the assessment of convergence.
%\subsection{The degenerate Dirichlet Trick (DDT)}
%\label{sec:ddt}
We can deal with this issue if we define a function $g()$ that transforms each categorical random variable $Z_j$ into a \textit{degenerate Dirichlet} distributed random variable, i.e., $Y_j=g(Z_j)$. 

Figure \ref{fig:cat2deg} illustrates this transformation using as example a random variable $Z$ with three possible outcomes $R_X \in \{1,2,3\}$. The probability is assigned to each outcome corresponding to $\eta_1,\eta_2$, and $\eta_3$, respectively. %Hence we say that $Z \sim Categorical(\eta)$, and $\eta=[\eta_1,\eta_2,\eta_3]$
The mapping $g()$ transforms $Z$ into a random variable $Y$ distributed according to degenerate Dirichlet distribution with parameters $\eta$, where $\eta=[\eta_1,\eta_2,\eta_3]$. %We conjecture the existence of $g(Z_j)$ for any categorically distributed random variable $Z_j$. 
The degenerate Dirichlet distribution is a special case of the Dirichlet distribution, in which all its probability mass is located at the only possible outcome $\eta$. %If the unique realization of the degenerate Dirichlet distribution corresponds to $\eta_j$, then 
The parameters of the degenerate Dirichlet distribution correspond to $\lim_{\alpha \to\infty} Dirichlet(\alpha\eta)$.  In summary:

$Y=g(Z) \sim deg$-$Dir(\eta)$ if $Z \sim Categorical(\eta)$.

%-- one is a multiple sampling expected value of the other --

%There is an strong connection between the categorical distributions and the degenerate Dirichlet distributions. . In effect, the only possible outcome of the degenerate Dirichlet corresponds to the parameters of the corresponding categorical distribution. From a generative perspective, sampling from a categorical distribution is equivalent to sampling from the categorical distribution generated by the degenerated distribution. The difference although subtle, it is important. 
%
%We transform the categorical distributions into degenerate Dirichlet distributions with the justification that there is a strong connection between both distributions. In effect, the only possible outcome of the degenerate Dirichlet corresponds to the parameters of the corresponding categorical distribution. From a generative perspective, sampling from a categorical distribution is equivalent to sampling from the categorical distribution generated by the degenerated distribution. The difference although subtle, it is important. 

%Formally, the  trick consists in defining the random variables $Z$ with the degenerate Dirichlet distribution that yields the conditional distributions, as opposed to using the conditional distributions themselves. Using the trick, the summations that give rise to the conditional distributions simplify greatly.

We apply the transformation to each of the random variables $Z_j$ as follows:

%%This Equation is correct and not easy to prove. The equation below is much safer
%\begin{align}
%~~~~~~~~Y_j &\sim g(Z_j) \implies f(Y_j)=g(f(Z_j)) =f(g(Z_j)) \nonumber\\
% f(Y_j)&{=}  \hspace{-0.2cm}{\int\displaylimits_{\eta_{-j} \in R_{Y_{-j}}}}\hspace{-0.3cm}f(Y_j|Y_{-%j}=\eta_{-j})\hspace{-0.2cm}\prod^{\textbf{M}}_{m=1,m \neq j}\hspace{-0.1cm} f(Y_m=\eta_m) ~dR_{Y_{-j}} \\
%&= f(Y_j|Y_{-j}=\eta_{-j})
%\label{eq:tractable}
%\end{align}

\begin{align}
~~~~~~~~~Y_j &\sim g(Z_j) \implies f(Y_j)=g(f(Z_j)) =f(g(Z_j)) \nonumber\\
 f(Y_j)&{=}  \hspace{-0.2cm}{\int\displaylimits_{\eta_{-j} \in R_{Y_{-j}}}}\hspace{-0.3cm}f(Y_j|Y_{-j}=\eta_{-j})f(Y_{-j}=\eta_{-j}) ~dR_{Y_{-j}} \\
&= f(Y_j|Y_{-j}=\eta_{-j})
\label{eq:tractable}
\end{align}

\vspace{-0.01cm}

Under the transformation, the summations in Equation \ref{eq:compoundlda} become a set of integrals, as we are now compounding continuous distributions. In addition, we note that the density of $Y_{-j}$ will \textit{only} be equal to one when it is evaluated at $\eta_{-j}$, i.e.,  $f(Y_{-j}{=}\eta_{-j})=1$. Hence, Equation 6 \textit{only} has values different than zero when %all of the random variables Y is assigned to its parameters 
$Y_{-j}=\eta_{-j}$. This leads to a considerable simplification. The solution then becomes tractable, as presented in Equation \ref{eq:tractable}.


%\begin{equation}
%\label{eq:tractable}
%f(Z_j) = f(Z_j|Y_{-j}=\eta_{-j},\textbf{X})\prod^{|\textbf{X}|}_{m=1} \cancelto{1}{f(Y_m=\eta_m)}+\sum_{z_1 = \eta_1} \dots \sum_{z_n = \eta_n} f(Z_0|Z_{-0},\textbf{X})\prod^{\textbf{|X|}}_{j=1} \cancelto{0}{f(Z_j=z_j)}
%\end{equation}

As a result, the substitution algorithm in conjunction with the mapping $g()$ overrides $D_{x^{(d)}_j}$, $W_{x^{(w)}_j}$, and $N_j$ of LDA-CGS (Equation \ref{eq:factors}) as follows:
\vspace{-0.01cm}

\begin{gather}
\begin{align}
D_{x^{(d)}_j}={\sum_{m=1,m\neq j}^{M}}\mathds{1}(x^{(d)}_j=x^{(d)}_m)*\eta_m ~~;~~ N_j={\sum_{m=1,m\neq j}^{M}}\eta_m\nonumber
\end{align}\\
W_{x^{(w)}_j}={\sum_{m=1,m\neq j}^{M}}\mathds{1}(x^{(w)}_j=x^{(w)}_m)*\eta_m 
\label{eq:dgmequations}
\end{gather}
%\vspace{-0.01cm}
where $\eta_m$ corresponds to the realization of the random variable $Y_m$. Upon convergence, the parameters are estimated from the following equations:
\begin{equation}
\label{eq:ldarcaparams}
\hat{\theta_{x^{(d)}_j}} \propto  (D_{x^{(d)}_j}+ \alpha) ~;~~ \hat{\phi_{x^{(w)}_j}} \propto (W_{x^{(w)}_j}+\beta)
\end{equation}

Formally, we name this process
%conjunction 
as recursively compound allocation (RCA). 
Algorithm \ref{alg:ldarca} summarizes the main steps of applying RCA to inference of LDA.


%\begin{figure*}[ht]
%\begin{align}
%\resizebox{0.5\textwidth}{!}{
%~~~~~Y^r_j,Y^c_j &\sim g(Z^r_j,Z^c_j) \implies f(Y^r_j,Y^c_j) = g(f(Z^r_j,Z^c_j)) = f(g(Z^r_j,Z^c_j)) = \nonumber\\
 %f(Y^r_j,Y^c_j)&{=}  \hspace{-0.2cm}{\int\displaylimits_{\eta_{-j} \in R_{Y^r_{-j},Y^c_{-j}}}}\hspace{-0.3cm}f(Y^r_j,Y^c_j|Y^r_{-j},Y^c_{-j}=\boldsymbol{\eta_{-j}})\hspace{-0.2cm}\prod^{\textbf{M}}_{m=1,m \neq j}\hspace{-0.1cm} f(Y^r_m,Y^c_m=\boldsymbol{\eta_m}) ~dR_{Y^r_{-j},Y^c_{-j}} \\
%&= f(Y^r_j,Y^c_j|Y^r_{-j},Y^c_{-j}=\boldsymbol{\eta_{-j}})
%\label{eq:tractabledt2b}
%\end{align}
%\end{figure*}


%\begin{equation}
%\resizebox{0.5\textwidth}{!}{$\sum_{q_\mathrm{total}=0}^{q_A+N_A+q_B+N_B-2}\left(\sum_{q_A=0}^{q_\mathrm{total}}\left(\binom{q_A+N_A-1}{q_A}\binom{q_B+N_B-1}{q_B}\right)\right)x^{q_\mathrm{total}}$}
%\end{equation}


%Figure \ref{fig:difference} illustrates the main difference between LDA-CGS and LDA-DGM by comparing their algorithmic differences.
\begin{algorithm}[b]
\begin{algorithmic}[1]
  \STATE \textbf{Input} Hyperparameters $K,\alpha,\beta$, dataset $\textbf{X}$, convergence threshold $\epsilon$
  \STATE Initialize $f(Y_j|Y_{-j}), ~\forall j \in 1 \cdots M$, and set initial iteration $i=1$
  \WHILE{marginal densities have not converged}
    \FOR{$j \in 1 \dots M$}
      \STATE  $Y_j^{i} \sim f(Y^{i}_j|Y^{i}_{<j},Y^{i-1}_{>j})$ from Equation \ref{eq:tractable} 
      %when using the degenerate Dirichlet trick
    \ENDFOR
    \STATE Converge if distance($f(Y_j^{i}),f(Y_j^{i-1})$) $ \leq \epsilon$
    \STATE $i=i+1$
  \ENDWHILE
% \STATE Estimate the parameters $\hat{\theta}$, $\hat{\phi}$ from Equation \ref{eq:ldadgmparams} when using the degenerate Dirichlet trick
\STATE Estimate $\hat{\theta}$ and $\hat{\phi}$ using Equation \ref{eq:ldarcaparams}.
 \RETURN $\hat{\theta}$, $\hat{\phi}$
\end{algorithmic}
\caption{Recursively Compound Allocation for LDA}
\label{alg:ldarca}
\end{algorithm}

As shown in Equation \ref{eq:factors} and \ref{eq:dgmequations}, the relationship between CGS and RCA is intuitive. 
It is clear that the calculation for the posterior density has transformed the caching for samples $z_j$ from the posterior distribution into the caching of the parameters $\eta_j$ for the posterior distribution. 
%To compute the posterior, LDA-DGM-DDT must cache the parameters of the posterior distribution for each document-word pair in the dataset. This, as opposed to caching a topic realization from the posterior distribution. 
The interpretation is that RCA assigns a mixture distribution over topics to each observed document-word pair, while in CGS the distribution is used to sample a single topic label. 
As a consequence, RCA provides a more flexible learning strategy for topic assignment compared to CGS.

%In probabilistic terms, 
During inference process,
the function $g()$ has transformed the vanilla LDA with categorical latent variables into a tractable model with degenerate Dirichlet latent variables. Because Dirichlet distributions sample over a probability simplex, this transformation is responsible for empowering LDA with soft-topic assignments. 
%In addition, we may highlight that, by introducing the function $g()$, which can transform a variable from categorical distribution to degenerate Dirichlet distribution, we have extended the basic topic models, and developed a new flexible topic model, where each exact topic assignment is replaced by the topic mixture assignment. 
In this way, the posterior of RCA is clearly different from the posterior of CGS. Thus,  
%Arguably, 
the new method RCA could perhaps lead to improved predictive performance for the inference of LDA compared to CGS. 
This justifies the differences in predictive perplexity in the experiments (See Section 6.2).




%%May not be technically correct
%Note that, different from the estimation for the parameters done by samples in LDA-CGS \cite{ldacgs}, in RCA, the parameters can be computed as a function of distributions.


%2018!!!
%With respect to the parameter estimation presented in Equations \ref{eq:ldacgsparams} and \ref{eq:ldadgmparams}, we observe in Equation \ref{eq:ldacgsparams} that the parameter estimation is based on counting samples which is constrained to be an integer-valued estimation. In contrast, Equation \ref{eq:ldadgmparams} shows that we estimate $\theta$ and $\phi$ from adding $\eta$ which corresponds to a more granular estimation based on real values.

%In addition, RCA has a guaranteed convergence, assessment of convergence and direct estimation of the marginal distributions $p(Y_j)$ and the parameters $\theta$ and $\phi$. However, we emphasize that the function $g()$ that casts a categorical distribution into a degenerate Dirichlet makes a transformation of LDA model into a model where topic assignments are replaced by topic mixture assignments and therefore the posterior of RCA does not correspond to the posterior of LDA-CGS. This further justifies the difference in predictive perplexity. Arguably, LDA with topic mixture assignments is a better modeling approach than the standard LDA.

\subsection{Applying RCA to Dual Topic Models}

We note that, in addition to latent Dirichlet allocation (LDA), RCA can be also applied to inference of other probabilistic topic models, such as dual topic model (DTM) \cite{dt2b}, relational topic model \cite{RTM}, and author-topic model \cite{atm}, etc.
%To further clarify how to apply the proposed method, we turn our attention to applying RCA to another probabilistic model. 
%In this case, we choose Dual Topics to Bicluster model (DT2B) because 
In contrast to many other topic models,
%such as the Relational Topic Model and the Author-Topic model, 
DTM models the pair-wise dependency between two types of latent topics \cite{dt2b}.
In this section, we turn our attention to applying RCA to DTM, and may shed some light on the inference procedure of such kind of topic models.


DTM takes as input a co-occurrence data matrix that underlies the inter-relationship between \textit{row} and \textit{column} variables, e.g., user-location matrix where each entry means the number of times a user (row) visited a location (column). 
Then, it extracts the row-topics $Z^r$ or distribution over the rows of the co-occurrence matrix, the column-topics $Z^c$ or distribution over the columns of the matrix, and the joint distribution of both column and row topics. 
This joint distribution models the dependency between the two types of topics. Therefore, we cannot transform $Z^r$ or $Z^c$ independently into $Y^r$ or $Y^c$ as done in LDA.

To apply RCA to DTM, we first derive the conditional posterior of CGS for DTM in Equation \ref{eq:dt2bcgs}:

\begin{gather}
f(Z^r_j,Z^c_j|Z^r_{-j}{=}z^r_{-j},Z^c_{-j}{=}z^c_{-j}) \propto \nonumber\\
\frac{(D_{x^{(d)}_j}+ \beta^r)}{(N^r_j+R\beta^r)} \dfrac{(W_{x^{(w)}_j}+\beta^c)}{(N^c_j+C\beta^c)}(P_j + \alpha)
\label{eq:dt2bcgs}
\end{gather}
where $R$ and $C$ are the numbers of rows and columns in the input matrix respectively, and the following are count vectors computed using the indicator function $\mathds{1}()$:
\begin{gather}
D_{x^{(d)}_j}={\sum_{m=1,m\neq j}^{M}}\mathds{1}(x^{(d)}_j=x^{(d)}_m)*z^r_m\nonumber\\
W_{x^{(w)}_j}={\sum_{m=1,m\neq j}^{M}}\mathds{1}(x^{(w)}_j=x^{(w)}_m)*z^c_m\nonumber\\
P_j{=}{\sum_{m=1,m\neq j}^{M}}{z^r_m}^\intercal . z^c_m\nonumber \\
N^r_j{=}{\sum_{m=1,m\neq j}^{M}}z^r_m  ~;~ N^c_j{=}{\sum_{m=1,m\neq j}^{M}}z^c_m
\label{eq:factors_dt2b}
\end{gather}


%To apply RCA effectively, 
We need to maintain the dependency between the two types of topics when mapping the joint distribution of the random variables $Z^r$ and $Z^c$ to the random variables $Y^r$ and $Y^c$. This is shown in Equation \ref{eq:tractabledt2b}

%%This belongs to RCA-DT2B:
%\begin{figure*}[ht]
\begin{gather}
Y^r_j,Y^c_j \sim g(Z^r_j,Z^c_j) \implies f(Y^r_j,Y^c_j) = f(g(Z^r_j,Z^c_j)) = \nonumber \\
\hspace{-0.1cm}{\int\displaylimits_{\eta_{-j} \in R_{Y^r_{-j},Y^c_{-j}}}}\hspace{-0.8cm}f(Y^r_j,Y^c_j|Y^r_{-j},Y^c_{-j}{=}\boldsymbol{\eta_{-j}}) f(Y^r_{-j},Y^c_{-j}{=}\boldsymbol{\eta_{-j}}) dR_{Y^r_{-j},Y^c_{-j}} \nonumber \\
= f(Y^r_j,Y^c_j|Y^r_{-j},Y^c_{-j}=\boldsymbol{\eta_{-j}})
\label{eq:tractabledt2b}
\end{gather}
%\end{figure*}


Note that $\boldsymbol{\eta}$ does no longer correspond to the parameters of a degenerate Dirichlet distribution as in the case of LDA shown in Equation \ref{eq:tractable}. 
Instead, $\boldsymbol{\eta}$ corresponds to a bivariate degenerate Dirichlet distribution.
%, and so we use bold font to remark this. 
To obtain the marginal density of $Y^r$ and $Y^c$, we can integrate $\boldsymbol{\eta}$ as shown in Equation \ref{eq:etas}.

\hspace{-0.1cm}
\begin{align}
\eta^r_j = \sum_{k_c}^{Kc} \boldsymbol{\eta_j} ~~~; ~~~\eta^c_j = \sum_{k_r}^{Kr} \boldsymbol{\eta_j}
\label{eq:etas}
\end{align}

As a result, the posterior equation of DTM-RCA replaces the values of $z^r$ presented in Equation \ref{eq:factors} for $\eta^r$. 
Similarly, RCA replaces the values of $z^c$ for $\eta^c$ for the factors $D_{x^{(d)}_j}$, $W_{x^{(w)}_j}$, $N^r_j$ and $N^c_j$. The factor $P_j$ depends on the joint assignment of $Y_j^r$ and $Y_j^c$. Therefore, the factor $P$ is computed as:

\hspace{-0.1cm}
\begin{align}
P_j={\sum_{m=1,m\neq j}^{M}}{\boldsymbol{\eta_m}}
\end{align}
%Finally, the parameters of RCA-DT2B can be estimated as  follows

%\begin{equation}
%\label{eq:ldadgmparams}
%\hat{\theta_{x^{(d)}_j}} \propto  (D_{x^{(d)}_j}+ \alpha) ~;~~ %\hat{\phi_{x^{(w)}_j}} \propto (W_{x^{(w)}_j}+\beta)
%\end{equation}


%\section{Discussion}


The flexibility in topic assignment by RCA results in improved predictive performance, as shown empirically in Section \ref{sec:exp}. Moreover, the additional key benefits of RCA are threefold: 1) RCA has a guaranteed convergence; 2) It is allowed to assess the status of convergence; and 3) In RCA, we can directly compute the marginal distributions $p(Y_j)$ and the parameters of the topic models


%The following was moved to after the explanation of LDA-RCA
%In addition, we may highlight that, by introducing the function $g()$, which can transform a variable from categorical distribution to degenerate Dirichlet distribution, we have extended the basic topic models, and developed a new flexible topic model, where each exact topic assignment is replaced by the topic mixture assignment. In this way, the posterior of RCA is clearly different from the posterior of CGS. Arguably, the new model could perhaps lead to better modeling performance compared to the standard LDA. This justifies the differences in predictive perplexity (See Section 6.2).
 
%**WHAT MODELS CAN BE APPLIED**
%- categorical latent variable
%- known collapsed gibbs sampler equation

%\subsection{Differences between DGM-LDA and DGM-LDA-DDT}


%Analytical solvability
%Flexibility
%Assessment of convergence


%DGM-LDA-DDT inherits the benefits of DGM-LDA, that is, guaranteed convergence, assessment of convergence and direct estimation of the marginal distributions $p(Z_j)$ and parameters $\theta$ and $\phi$. However, the function $g$ that casts a categorical distribution into a degenerate Dirichlet makes a transformation of LDA model into a different model and therefore the posterior of DGM-LDA-DDT does not correspond to the posterior of DGM-LDA. 

%Empirically, we show in section \ref{sec:exp} that this transformation is beneficial as shown by an improvement in predictive accuracy. LDA-DGM-DDT is a more flexible model because each row in the dataset is no longer assigned to a topic drawn by a categorical distribution but to a mixture of topics drawn from the degenerate-Dirichlet distribution. In addition, the estimation of the parameters $\theta$ and $\phi$ is more granular. This is due to the fact that the values $D_{x^{(d)}_j}$ and $W_{x^{(w)}_j}$ are mapped from an integer space in Equation \ref{eq:ldacgsparams}-- because they represent countings, to a real space in Equation \ref{eq:ldadgmparams} -- because they represent sums of parameters residing on the real space. %The following are the equations for estimating the parameters in LDA-DGM using DDT:



%As in Gibbs sampling, the estimation converges to the true values of the parameters as the iterations grow to infinity. However, different from Gibbs sampling, the convergence assessment can be simply done by checking the changes of parameter values in-between iterations.%The difference between the two models is given by 
%sum sum sum = sum of distros
%Note that representing the posterior with a categorical distribution leads to a different result.
%Section \ref{sec:exp} shows the benefits in predictive perplexity obtained by using DGM in conjunction with the Dirichlet trick.

% Comment on time complexity 

%The fact that both approaches differ will explain the difference in parameter estimation obtained by both algorithms. 

%\subsection{The mixture of experts }

%\subsection{Applicability to other models}

%In this work, we only explore models where DGM is used in conjunction with the Degenerate Dirichlet trick. So, when we refer to DGM, we are implying that we are also using the trick. DGM provide us with a theoretical foundation to perform inference in a family of latent topic models where 1) standard collapsed Gibbs sampling applies and 2) all the posterior conditional distributions are categorical. Examples of these include the Relational Topic Model, Hidden Markov Model, Supervised LDA, Correlated Topic Model and the Collaborative Topic Model.


\section{Proof for Convergence of RCA}
\label{subsec:proof}

Without much loss of generality, it is sufficient to show the equivalence between RCA and Gibbs sampling using the case of two joint Bernoulli random variables $X$ and $Y$. We note that the proof for the convergence of Gibbs sampling in \cite{casella} directly leverages compounded distributions rather than sampling. 
In the paper, they showed that the desired marginal distribution $p(X)$ corresponds to the stationary distribution of a Markov chain with transition matrix $A_{X|X}=A_{Y|X}A_{X|Y}$, where $A_{Y|X}$ and $A_{X|Y}$ are the conditional densities:
\vspace{-0.1cm}
\[A_{Y|X}=f_{Y|X}(y) ~;~~ A_{X|Y}=f_{X|Y}(x)\]

Therefore, the approximated density of the marginal distribution at the $i^{th}+1$ iteration can be found from the approximated marginal distribution:
\vspace{-0.1cm}
\begin{equation}
\label{eq:xchain}
f_{X^{i+1}}(x)=f_{X^i}(x)f_{Y^i|X^i}(y)f_{X^i|Y^i}(x) 
\end{equation}

As we run for more iterations, the approximated marginal distributions approach the target marginal distributions, i.e., $\lim_{i\to\infty} f_{X^i}(x) \to f_{X}(x)$. The connection with RCA follows, 
as it can be observed that the intermediary steps of the Equation \ref{eq:xchain} correspond to the compounding process. 
This can be checked by proposing that the combination of the first two factors corresponds to the approximated marginal $f_{Y^i}(y)$.

\begin{equation}
\label{eq:fx}
f_{X^{i+1}}(x)=f_{Y^i}(y)f_{X^i|Y^i}(x) 
\end{equation}
\vspace{-0.25cm}
\begin{equation}
\label{eq:fy}
f_{Y^i}(y)=f_{X^i}(x)f_{Y^i|X^i}(y)
\end{equation}

Following the same rule, we propose $f_{X^i}(x)=f_{Y^{i-1}}(x)f_{X^{i-1}|Y^{i-1}}(y)$. We show that the proposition about $f_{Y^i}(y)$ is correct by plugging the proposition of $f_{X^i}(x)$ into the above equation. Then we end up with:

\[f_{Y^i}(y)=f_{Y^{i-1}}(x)f_{X^{i-1}|Y^{i-1}}(y)f_{Y^i|X^i}(y)\]


This corresponds to the Markov chain equation whose stationary distribution targets the marginal distribution of $f_{Y}(y)$. Thus, the proposition for $f_{Y^i}(y)$ is correct. The same argument can be used to show that the proposition for $f_{X^i}(x)$is also true.

Finally, we notice that the evaluation of Equations \ref{eq:fx} and \ref{eq:fy} corresponds to compounding the conditional distributions presented in Algorithm \ref{alg:ldarca}.
\vspace{-0.1cm}
\[f_{Y^{i+1}}(y')=\sum_{x' \in R_X}f_{X^i}(x')f_{Y|X}(y'|x') ~,~~\forall y' \in R_Y\]
\vspace{-0.1cm}
\[f_{X^{i+1}}(x')=\sum_{y' \in R_Y}f_{Y^i}(y')f_{X|Y}(x'|y') ~,~~\forall x' \in R_X\]

By using the degenerate Dirichlet distribution, we transform the target density distributions to be $f_{g(X)}$ and $f_{g(Y)}$, so that the method is guaranteed to converge using the following equations:
\vspace{-0.1cm}
\[f_{g(Y^{i+1})}(y')=\int_{x' \in R_{g(X)}}f_{g(X^i)}(x')f_{Y|g(X)}(y'|x') ~,~~\forall y' \in R_Y\]
\vspace{-0.2cm}
\[f_{g(X^{i+1})}(x')=\int_{y' \in R_{g(Y)}}f_{g(Y^i)}(y')f_{X|g(Y)}(x'|y') ~,~~\forall x' \in R_X\]

Although the convergence may be biased to a different marginal distribution, we emphasize that this is perhaps beneficial in topic models such as latent Dirichlet allocation.




==> 6.VI.tex <==
\section{Connection with Mean Field Variational Inference}

Variational inference approximates the posterior $P(Z_1,\cdots,Z_m|\textbf{X})$ using an optimization-based approach. 
The solution is given by fitting a proposed distribution $q(Z)$ to the posterior as measured by the Kullback-Leibler (KL) divergence. 
The relationship between $q(Z)$ and $P(Z|\textbf{X})$ is given as follows:

\begin{equation}
log~p(\textbf{X}) = ELBO(q) +  D_{KL}(q_{\gamma}(Z)||p(Z|\textbf{X})),
\end{equation}
where
\begin{center}
$ELBO(q)=\mathbb{E}_q\left[log~p(Z,\textbf{X})\right]+\mathbb{E}_q\left[log~q(Z)\right] $.
\end{center}
 
 
Since the evidence $P(\textbf{X})$ is strictly positive and independent of the latent variables $Z$, maximizing the $ELBO(q)$ is equivalent to minimizing the KL divergence. %the optimization problem is often solved by maximizing the ELBO. 
A common algorithm used to maximize the ELBO is coordinate ascent variational inference (CAVI) presented in Algorithm \ref{alg:cavi} \cite{reviewvi}.

\begin{algorithm}
\begin{algorithmic}[1]
  \STATE \textbf{Input} A model $p(\textbf{X},Z)$, a dataset $\textbf{X}$
  \STATE \textbf{Initialize} Variational factors $q_j(Z_j)$
  \WHILE{ELBO(q) has not converged}
  	\FOR{$ j\in 1 \dots \textbf{M}$}
      \STATE  Set $q_j(Z_j) \propto exp\left[\mathbb{E}_{q_{-j}}\left[log~p(Z_j|Z_{-j},\textbf{X})\right]\right]$
    \ENDFOR
   \STATE Compute $ELBO(q)=\mathbb{E}_q\left[log~p(Z,\textbf{X})\right]+\mathbb{E}_q\left[log~q(Z)\right]$
  \ENDWHILE
\RETURN $q(Z)=\prod_{j=1}^{M} q_j(Z_j)$
\end{algorithmic}
\caption{Coordinate ascent variational inference (CAVI)}
\label{alg:cavi}
\end{algorithm}

The relationship between variational inference and the proposed method RCA appears, %can be noted 
if we propose $q_j(Z_j) \sim deg$-$Dir(\eta_j)$ to approximate the posterior of RCA presented in Equation \ref{eq:tractable}. Assuming the density of $q_j(Z_j)$ as $f_{Z_j}(z)$, step 5 of Algorithm \ref{alg:cavi} turns to be:

\begin{equation}
\label{eq:compound}
q_j(Z_j) \propto exp \left(\int \cdots \int  log~f_{Z_j|Z_{-j},\textbf{X}}(z)\prod^{\textbf{M}}_{m=1,m\neq j} f_{Z_j}(z) d_{z{-j}} \right)
\end{equation}

%If we assume the density $f_{Z_j|Z_{-j}}(z|\eta_j)$ to be deg-Dirichlet distributed.
The integrals of Equation \ref{eq:compound} are different than zero only when $Z_j=\eta_j ~\forall j \in 1 \ldots M$. %Coincidentally $f_Z(\eta)=1$. 
Therefore, we obtain that:
$$q_j(Z_j) = exp\left(log\left(f_{Z_j|Z_{-j}}(z|\eta_j)\right)\right)$$



%In conclusion, if we propose $q_j(Z_j) \sim deg_Dir$ to approximate the posterior of DGM-DDT-LDA presented in Equation \ref{eq:tractable}. Then, CAVI algorithm \ref{alg:cavi} turns out to be identical to DGM-DDT algorithm \ref{alg:dgm}. Because in this scenario CAVI converges to the same objective of the Gibbs method, we observer that CAVI does a perfect approximation to the posterior of DGM-DDT when we initialize the variational family with degenerate-Dirichlet distributions. This observation may be used to transfer existing advantages of the mean-field variational inference algorithm into the Gibbs sampling framework.


%In conclusion, Several latent models have as commonality the fact that their posterior conditional distributions are discrete. Discrete distributions have a property of 'closure'. Under certain conditions a compound of a discrete distribution with discrete random variables yields a discrete density. With the use of this property, the loop of DGE can continue without yielding compound distributions that become incrementally complex.




\begin{table*}[!t]
\caption{Automatic topic coherence results of LDA inferred by RCA or CGS, where the RCA results are highlighted in grey.}
\label{tab:topiccoherence}
  \centering
  \setlength\tabcolsep{7pt} 
  
  %\begin{tabular}{c@l^c>{\scriptsize}^c^c>{\scriptsize}^c^c>{\scriptsize}^c}
  \bgroup
\def\arraystretch{1.2}
  \begin{tabular}{c@l^c^c^c|^c^c|^c^c}
    \toprule
     \multirow{2}*{Dataset} &  \multirow{2}*{N} &   \multirow{2}*{Method} &  \multicolumn{2}{c}{LCP} &  \multicolumn{2}{c}{PMI} &  \multicolumn{2}{c}{NPMI} \\
            &  & & mean &  max , min & mean & max , min & mean & max , min \\
    \midrule
    \multirow{6}*{NIPS} %rotatebox{90}{}                
             &                \multirow{2}*{10} & CGS & -6.662 & -6.08 , -6.96 &          0.841 & 1.20 , 0.55 &          0.057 & 0.09 , 0.04 \\
             &    & \rowstyle{\cellcolor{hcolor}} RCA &  \textbf{-6.588}& -6.17 , -6.93 & \textbf{0.942} & 1.28 , 0.59 & \textbf{0.063} & 0.08 , 0.04\\
             &                \multirow{2}*{20} & CGS &  -6.682 & -6.14 , -6.92 &          0.806 & 1.03 , 0.55 &          0.054 & 0.07 , 0.04 \\
             &    & \rowstyle{\cellcolor{hcolor}} RCA &  -6.619 & -6.14 , -6.98 &          0.879 & 1.15 , 0.58 &          0.059 & 0.07 , 0.04\\
             &                \multirow{2}*{50} & CGS &  -6.687 & -6.17 , -6.86 &          0.759 & 0.91 , 0.56 &          0.051 & 0.06 , 0.04\\
             &    & \rowstyle{\cellcolor{hcolor}} RCA &  -6.641 & -6.16 , -6.93 &          0.801 & 0.98 , 0.58 &          0.054 & 0.06 , 0.04 \\
            % &               \multirow{2}*{100} & CGS &  -6.695 & -6.22 , -6.84 &          0.737 & 0.85 , 0.58 &          0.050 & 0.06 , 0.042 \\
            % &    &\rowstyle{\cellcolor{hcolor}} RCA &  -6.646 & -6.19 , -6.96 &          0.758 & 0.92 , 0.59 &          0.051 & 0.06 , 0.043 \\
    \midrule
    \multirow{6}*{Lastfm}                      
             &               \multirow{2}*{10}  & CGS & -5.031 & -4.56 , -5.79 &          1.618 & 2.54 , 0.94 &          0.128 & 0.19 , 0.08 \\
             &    & \rowstyle{\cellcolor{hcolor}} RCA &\textbf{-4.993}& -4.52 , -5.70 & \textbf{1.692} & 2.38 , 1.15 & \textbf{0.133} & 0.18 , 0.09\\
             &               \multirow{2}*{20}  & CGS & -5.205 & -4.79 , -6.02 &          1.631 & 2.49 , 1.02 &          0.125 & 0.18 , 0.08 \\
             &    &\rowstyle{\cellcolor{hcolor}}  RCA & -5.236 & -4.78 , -6.04 &          1.689 & 2.33 , 1.13 &          0.129 & 0.18 , 0.09\\
             &               \multirow{2}*{50}  & CGS & -5.572 & -5.17 , -6.32 &          1.644 & 2.36 , 1.02 &          0.119 & 0.17 , 0.07 \\
             &    &\rowstyle{\cellcolor{hcolor}}  RCA & -5.601 & -5.17 , -6.56 & \textbf{1.692} & 2.30 , 1.06 &          0.122 & 0.17 , 0.08 \\
            %                \multirow{2}*{100} & CGS & -5.929 & -5.41 , -6.50 &          1.626 & 2.29 , 0.97 &          0.112 & 0.16 , 0.07 \\
            % &   & \rowstyle{\cellcolor{hcolor}} RCA & -5.955 & -5.43 , -6.79 &          1.673 & 2.29 , 1.02 &          0.115 & 0.16 , 0.07 \\
\midrule       
     \multirow{6}*{Movielens}
             &                \multirow{2}*{10} & CGS & -6.182 & -5.65 , -6.77 & \textbf{0.732} & 1.16 , 0.59 &          0.053 & 0.09 , 0.04 \\
             &    &\rowstyle{\cellcolor{hcolor}}  RCA & \textbf{-5.669} & -5.56 , -6.02 &          0.689 & 1.09 , 0.55 & \textbf{0.054} & 0.08 , 0.04 \\
             &                \multirow{2}*{20} & CGS & -6.198 & -5.74 , -6.66 &          0.724 & 1.08 , 0.63 &          0.053 & 0.08 , 0.04\\
             &    &\rowstyle{\cellcolor{hcolor}}  RCA & \textbf{-5.699} & -5.57 , -6.04 &          0.688 & 1.09 , 0.55 &          0.053 & 0.08 , 0.04 \\
             &                \multirow{2}*{50} & CGS & -6.231 & -5.78 , -6.57 &          0.723 & 1.01 , 0.63 &          0.052 & 0.07 , 0.04 \\
             &    &\rowstyle{\cellcolor{hcolor}}  RCA & -5.774 & -5.63 , -6.21 &          0.682 & 1.02 , 0.56 &          0.052 & 0.07 , 0.04\\
           % &               \multirow{2}*{100} & CGS & -6.273 & -5.81 , -6.52 &          0.713 & 0.94 , 0.64 &          0.051 & 0.08 , 0.04 \\
           % &    &\rowstyle{\cellcolor{hcolor}}  RCA & -5.845 & -5.70 , -6.30 &          0.677 & 0.95 , 0.58 &          0.051 & 0.07 , 0.04 \\
  \bottomrule
  \end{tabular}
  \egroup
\end{table*}



This equation makes CAVI (Algorithm \ref{alg:cavi}) become identical to RCA (Algorithm \ref{alg:ldarca}). In addition, because CAVI converges to the same objective of the Gibbs method, we notice that CAVI does a perfect approximation to the posterior of RCA when we initialize the variational family with degenerate-Dirichlet distributions. 
This observation may be potentially useful for transfering existing advantages of the mean-field variational inference algorithm into the Gibbs sampling framework.





==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios
		Code prettying (Michael D. Adams)
		Two-column formats now balance the last page (ACM request)
		

==> attemptderivem.tex <==
%https://www0.gsb.columbia.edu/faculty/mjohannes/PDFpapers/MCMCMLE_2006.pdf

In this paper we show that it is possible to derive a formula

$p(\Theta,Z,X) \propto \prod_{r=1}^R p(\Theta^{(r)},Z,X)$

prop means that there exist a constant to multiply
It makes sense that the constant increases as the number of replications grows

(maybe we ignore this fact and just multiply divide by 1/r)

$p(\Theta,Z,X) \propto \prod_{r=1}^R p(\Theta^{(r)},Z,X)$

r is the number of replications 

Since Z independent given theta (Eq 17)
$\int \prod p(z|\theta)p(\theta|\alpha) \times \int \prod p(y|\phi,z)p(\phi|\beta)$

(Eq 22)
\begin{table*}
\large
\begin{equation}
\lim_{r \to \infty} \dfrac{1}{r}
\prod_m \int 
	\dfrac{\Gamma(\sum_k \alpha_k)}{\prod_k \Gamma(\alpha_k)}
     \prod_k \theta^{\alpha_k-1+\sum_r c_{k^{(r)},m,*}}_{m,k} d\theta_m \times
\prod_k \int 
	\dfrac{\Gamma(\sum_j \beta_j)}{\prod_k \Gamma(\beta_k)}
     \prod_j \phi^{\beta_k-1+\sum_r c_{k^{(r)},m,*}}_{k,j}  d\phi_k
\end{equation}
\\
%(Eq 25)
\begin{equation}
\large
\prod_m \dfrac{\prod_k \Gamma( \sum_r c_{k^{(r)},m,*}+\alpha_k)}
              {\Gamma(\sum_k \sum_r c_{k^{(r)},m,*}+\alpha_k)}
\times
\prod_k \dfrac{\prod_j \Gamma( \sum_r c_{k^{(r)},*,j}+\beta_j)}
              {\Gamma(\sum_j \sum_r c_{j^{(r)},*,j}+\beta_j)}
\end{equation}
\\
%(Eq 27)
\begin{equation}
\large
 \dfrac{\prod_k \Gamma( \sum_r c_{k^{(r)},a,*}+\alpha_k)}
              {\Gamma(\sum_k \sum_r c_{k^{(r)},a,*}+\alpha_k)}
\times
\prod_k \dfrac{\prod_j \Gamma( \sum_r c_{k^{(r)},*,j}+\beta_{y_{a,b}})}
              {\Gamma(\sum_j \sum_r c_{j^{(r)},*,j}+\beta_j)}
\end{equation}
\\
However there are many counts for a single record. 

\end{table*}


(Eq 32)
\begin{equation}
\large
\propto 
\dfrac{
	\left( \sum_r c^{-(a,b)}_{z^{(r)}_{a,b},a,*} + \alpha_{z^{(r)}_{a,b}} \right) 
    \times 
    \left( \sum_r c^{-(a,b)}_{z^{(r)}_{a,b},*,y_{a,b}} + \beta_{y_{a,b}}  \right)} 
	{ \sum_r c^{-(a,b)}_{z^{(r)}_{a,b},*,*}+\sum_j \beta_{j}}
\end{equation}


other models where it is unclear how to use the Poisson sampler to estimate the topic assignments 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Update for replicated DTM:

The update for the $j^{th}$ row-column pair can be found as:
\begin{gather}
\label{eq:post1}
p'(Z_j,Y_j|Z^{(1)}_{-j} .. Z_{-j}^{(R)},Y^{(1)}_{-j} .. Y_{-j}^{(R)},X) \propto A*B*C\nonumber\\
A = \dfrac{ \left( \sum_r c^{-(a,b)}_{z^{(r)}_{a,b},*,*,y_{a,b}} + \beta_{y_{a,b}}  \right)} 
	{ \sum_r c^{-(a,b)}_{z^{(r)}_{a,b},*,*}+\sum_j \beta_{j}} \nonumber\\
B = \dfrac{ \left( \sum_r c^{-(a,b)}_{*,z^{(r)}_{a,b},*,y_{a,b}} + \beta_{y_{a,b}}  \right)} 
	{ \sum_r c^{-(a,b)}_{*,z^{(r)}_{a,b},*,*}+\sum_j \beta_{j}} \nonumber\\
C=  \sum_r c^{-(a,b)}_{z^{(r)}_{a,b},y,*,*} + \alpha_{z^{(r)}_{a,b}} 
\end{gather}


